Simply tell me how -- On Trustworthiness and Technology Acceptance of Attribute-Based Credentials

Attribute-based Credential Systems (ACS) have been long proposed as privacy-preserving means of attribute-based authentication, yet neither been considered particularly usable nor found wide-spread adoption, to date. To establish what variables drive the adoption of \ACS as a usable security and privacy technology, we investigated how intrinsic and presentation properties impact their perceived trustworthiness and behavioral intent to adopt them. We conducted two confirmatory, fractional-factorial, between-subject, random-controlled trials with a total UK-representative sample of $N = 812$ participants. Each participant inspected one of 24 variants of Anonymous Credential System Web site, which encoded a combination of three intrinsic factors (\textsf{provider}, \textsf{usage}, \textsf{benefits}) and three presentation factors (\textsf{simplicity}, presence of \textsf{people}, level of available \textsf{support}). Participants stated their privacy and faith-in-technology subjective norms before the trial. After having completed the Web site inspection, they reported on the perceived trustworthiness, the technology adoption readiness, and their behavioral intention to follow through. We established a robust covariance-based structural equation model of the perceived trustworthiness and technology acceptance, showing that communicating facilitating conditions as well as demonstrating results drive the overall acceptance and behavioral intent. Of the manipulated causal variables, communicating with simplicity and on the everyday usage had the greatest and most consistently positive impact on the overall technology acceptance. After earlier correlational empirical research on ACS technology acceptance, ours is the first research showing cause-effect relations in a structural latent factor model with substantial sample size.

==> Perceived_ABC_Trustworthiness-concordance.tex <==
\Sconcordance{concordance:Perceived_ABC_Trustworthiness.tex:Perceived_ABC_Trustworthiness.Rnw:%
1 23 1 50 0 1 5 219 1 1883 0}


==> condition_table.tex <==
\begin{table*}[htbp]
\centering
\caption{Experimental conditions and descriptives of trust and behavioral intention.} 
\label{tab:conditions}
\begingroup\footnotesize
\begin{tabular}{lllllllrrrrr}
  \toprule
\multirow{2}{*}{Survey} & \multirow{2}{*}{\textsf{provider}} & \multirow{2}{*}{\textsf{benefits}} & \multirow{2}{*}{\textsf{usage}} & \multirow{2}{*}{\textsf{simplicity}} & \multirow{2}{*}{\textsf{people}}
 & \multirow{2}{*}{\textsf{support}} & \multirow{2}{*}{$n$} & 
\multicolumn{2}{c}{\textsf{trust}} & \multicolumn{2}{c}{\textsf{bi}}\\
\cmidrule(l){9-10} \cmidrule(l){11-12}
&&&&&&&& $M$ & $\vari{SD}$ & $M$ & $\vari{SD}$\\
  \midrule
Intrinsic & Company & Privacy & Everyday & simple & photo & nosupport &  26 & 4.26 & 1.21 & 4.45 & 1.48 \\ 
  Intrinsic & Company & Privacy & Tech & simple & photo & nosupport &  31 & 4.52 & 0.88 & 4.54 & 1.08 \\ 
  Intrinsic & Company & User & Everyday & simple & photo & nosupport &  37 & 4.24 & 1.13 & 4.12 & 1.51 \\ 
  Intrinsic & Company & User & Tech & simple & photo & nosupport &  31 & 4.24 & 1.29 & 4.49 & 1.79 \\ 
  Intrinsic & Government & Privacy & Everyday & simple & photo & nosupport &  29 & 4.39 & 1.18 & 4.38 & 1.52 \\ 
  Intrinsic & Government & Privacy & Tech & simple & photo & nosupport &  39 & 4.16 & 1.01 & 4.63 & 1.36 \\ 
  Intrinsic & Government & User & Everyday & simple & photo & nosupport &  41 & 4.24 & 1.08 & 4.54 & 1.34 \\ 
  Intrinsic & Government & User & Tech & simple & photo & nosupport &  39 & 4.28 & 1.18 & 4.31 & 1.65 \\ 
  Intrinsic & University & Privacy & Everyday & simple & photo & nosupport &  27 & 4.57 & 0.86 & 4.47 & 1.31 \\ 
  Intrinsic & University & Privacy & Tech & simple & photo & nosupport &  40 & 4.67 & 0.92 & 4.40 & 1.41 \\ 
  Intrinsic & University & User & Everyday & simple & photo & nosupport &  36 & 4.07 & 0.93 & 4.45 & 1.25 \\ 
  Intrinsic & University & User & Tech & simple & photo & nosupport &  26 & 4.69 & 0.95 & 5.06 & 1.13 \\ 
  Presentation & none & User & Everyday & complex & nophoto & contact &  27 & 4.44 & 1.06 & 4.64 & 1.69 \\ 
  Presentation & none & User & Everyday & complex & nophoto & fullsupport &  40 & 4.35 & 0.87 & 4.33 & 1.38 \\ 
  Presentation & none & User & Everyday & complex & nophoto & nosupport &  35 & 4.14 & 0.94 & 3.90 & 1.21 \\ 
  Presentation & none & User & Everyday & complex & photo & contact &  32 & 4.38 & 1.10 & 4.28 & 1.46 \\ 
  Presentation & none & User & Everyday & complex & photo & fullsupport &  40 & 4.36 & 0.88 & 4.28 & 1.45 \\ 
  Presentation & none & User & Everyday & complex & photo & nosupport &  35 & 4.00 & 0.90 & 4.16 & 1.31 \\ 
  Presentation & none & User & Everyday & simple & nophoto & contact &  30 & 4.32 & 1.25 & 4.97 & 1.22 \\ 
  Presentation & none & User & Everyday & simple & nophoto & fullsupport &  43 & 4.28 & 1.27 & 4.58 & 1.37 \\ 
  Presentation & none & User & Everyday & simple & nophoto & nosupport &  46 & 4.05 & 0.97 & 4.46 & 1.25 \\ 
  Presentation & none & User & Everyday & simple & photo & contact &  33 & 4.60 & 0.87 & 4.65 & 1.22 \\ 
  Presentation & none & User & Everyday & simple & photo & fullsupport &  31 & 4.20 & 0.75 & 4.45 & 1.33 \\ 
  Presentation & none & User & Everyday & simple & photo & nosupport &  41 & 4.35 & 0.92 & 4.76 & 1.26 \\ 
   \bottomrule
\end{tabular}
\endgroup
\end{table*}


==> demographics.tex <==
\newcommand{\demoTableB}{
\begin{table}
\centering
\caption{Sample $N=835$}
\begin{tabular}{llll}
\toprule
 Class & Number & Class & Number\\
\midrule
\textbf{N} & 835\\
\textbf{Gender (\%)} & \\
Male & 402 (48.1)\\
Female & 426 (51.0)\\
Rather not say & 7 ( 0.8)\\
\addlinespace
\textbf{Age (\%)} & \\
Under 18 & 1 ( 0.1)\\
18-24 & 137 (16.4)\\
25-34 & 218 (26.1)\\
35-44 & 171 (20.5)\\
\addlinespace
45-54 & 117 (14.0)\\
55-64 & 145 (17.4)\\
65+ & 46 ( 5.5)\\
\textbf{Mothertongue (\%)} & \\
English & 817 (97.8)\\
\addlinespace
Arabic & 2 ( 0.2)\\
Greek & 3 ( 0.4)\\
Hindi & 1 ( 0.1)\\
Italian & 2 ( 0.2)\\
Polish & 1 ( 0.1)\\
\addlinespace
Portuguese & 1 ( 0.1)\\
Russian & 2 ( 0.2)\\
Spanish & 1 ( 0.1)\\
Tagalog & 1 ( 0.1)\\
Urdu & 1 ( 0.1)\\
\addlinespace
Other & 3 ( 0.4)\\
\bottomrule
\end{tabular}
}


\newcommand{\demoTable}{
\begin{table}
\centering
\caption{Sample Demographics ($N = 835$)}
\label{tab:demo}
\begin{subtable}[b]{0.49\columnwidth}
\subcaption{By Gender, Age}
\begin{tabular}{lr@{ }r}
\toprule
 & Overall & (\%)\\
\midrule
\textbf{Gender}& \\
Male & 402 & (48.1)\\
Female & 426 & (51.0)\\
Rather not say & 7 & ( 0.8)\\
\addlinespace
\textbf{Age} & \\
Under 18 & 1 &(0.1)\\
18-24 & 137 &(16.4)\\
25-34 & 218 &(26.1)\\
35-44 & 171 &(20.5)\\
\addlinespace
45-54 & 117 &(14.0)\\
55-64 & 145 &(17.4)\\
65+ & 46 & (5.5)\\
\bottomrule
\end{tabular}
\end{subtable}~
\begin{subtable}[b]{0.49\columnwidth}
\subcaption{By Mother Tongue}
\begin{tabular}{lr@{ }r}
\toprule
   & Overall\\
\midrule
\textbf{Mother Tongue} & \\
English & 817 & (97.8)\\
\addlinespace
Arabic & 2 &(0.2)\\
Greek & 3 &(0.4)\\
Hindi & 1 & (0.1)\\
Italian & 2 & (0.2)\\
Polish & 1 & (0.1)\\
\addlinespace
Portuguese & 1 & (0.1)\\
Russian & 2 & (0.2)\\
Spanish & 1 & (0.1)\\
Tagalog & 1 & (0.1)\\
Urdu & 1 & (0.1)\\
\addlinespace
Other & 3  & (0.4)\\
\bottomrule
\end{tabular}
\end{subtable}
\end{table}
}

==> expected_covariance.tex <==

\newcommand{\IUIPC}{\textsf{IUIPC}}
\newcommand{\FC}{\textsf{FC}}
\newcommand{\Trust}{\textsf{Trust}}
\newcommand{\Reliability}{\textsf{Reliability}}
\newcommand{\PrimaryUse}{\textsf{PrimaryUsefulness}}
\newcommand{\PrivacyUse}{\textsf{PrivacyUsefulness}}
\newcommand{\BI}{\textsf{BI}}
\begin{table*}
\centering
\caption{Expected co-variances and correlated errors based on instrument properties.}
\label{tab:covar}
\begin{tabular}{llp{10cm}}
\toprule
Construct & Variables & Reasoning\\
\midrule
\IUIPC & \textsf{IUIPC1}, \textsf{IUIPC2} & parallel measures both about the central role of consumer control.\\
\FC & \textsf{STFC1}, \textsf{STFC2} & both state ``I have the [resources/knowledge] to\dots'' dependent on the hidden variable of knowledge what is needed.\\
\Trust & \textsf{STT1}, \textsf{STT2} & parallel measures, mentioning largely equivalent statements about trust and trustworthiness.\\
\PrimaryUse & \textsf{STPE2}, \textsf{STPE3} & \textsf{STPE2} and \textsf{STPE3} mention ``tasks'' filled by participants with meaning.\\
\PrivacyUse & \textsf{TAU2}, \textsf{TAU3} & parallel measures about increasing privacy protection.\\
\BI & \textsf{STBI3}, \textsf{STBI4} & Both statements about predictions of the future.\\
\midrule
\Trust & \Reliability, \Trust & Both latent variables similar items in getting the job done.\\
\bottomrule
\end{tabular}
\end{table*}


==> manipulations_table.tex <==
\begin{table*}
\centering
\caption{Content used for intrinsic interventions.}
\label{tab:manipulations_content}
\begin{tabular}{llp{12cm}}
\toprule
Level  & Variant & Content \\
\midrule
\multicolumn{3}{c}{Variable: \textsf{provider}}\\
\midrule
\textsf{government} & &
At the Government Digital Service our core purpose is to help government work better for everyone in the UK. We do this by building technological services and enforcing digital standards. We value innovation and delivery of user-focused services with the goal of positively impacting individuals, technologies and government.\\
\addlinespace
\textsf{company} & &
At IBM our core purpose is to promote our client?s success. We do this by offering high quality technological and business services in the UK and also around the world. We value intelligence, reason and science with the goal of positively impacting business, society and the human condition.\\
\addlinespace
\textsf{university} & &
At [anonymized] University our core purpose is to advance education. We do this through high quality teaching and research [...]. We value academic excellence, innovation and creativity with the goal of positively impacting individuals, organisations and society.\\
\textsf{none} & &
[The system] is a new product that lets users give online service providers access to their personal information in a safe and secure way.\\
\midrule
\multicolumn{3}{c}{Variable: \textsf{usage}}\\
\midrule
\textsf{everyday} & Intrinsic &
The system gives you the ability to prove personal details to service providers. For instance, you can prove that you are older than the minimum age to buy a product. You can also prove your membership of organisations. You receive a credential on a collection of your personal details which you can then selectively prove to a service provider. You can have multiple identities and can choose which details you wish to disclose. You can verify your identity without revealing details such as your name, nationality and date of birth.\\
\addlinespace
& Presentation &
Online providers often require their users to confirm certain information to make sure they eligible for their content. This information can range from phone numbers to home addresses. With [this system], users can choose the information they would like to reveal to service providers. Information that the user does not want the provider to have access to would remain private and protected. \\
\addlinespace
\textsf{tech} & &
The system provides its users with a credential. They can use this to prove to service providers that they satisfy the policy to use a service or buy a product. Collaborating with an Issuer organisation they receive a credential. The credential is on a set of attributes such as their name, nationality or date of birth. As such, a credential is a digital signature on a list of attribute-value pairs. The user has access to software that takes their credential and provides proof that their attributes fulfil a service provider's policy without revealing the attributes.\\
\midrule
\multicolumn{3}{c}{Variable: \textsf{benefits}}\\
\midrule
\textsf{user} & Intrinsic &
Prove your age for media or buying alcohol, without disclosing your date of birth or other data
Prove your memberships to gyms, cinemas and universities without being traceable
Benefit from your favourite services without the provider being able to profile you\\
\addlinespace
 & Presentation &
 Users are also able to let providers verify their information without giving them direct access to it. This means a user would be able to provide proof to a company that they are over a certain age without telling the company their exact birthdate.\\
\addlinespace
\textsf{privacy} & &
Protect privacy by minimising the data that is disclosed to service providers
Enable multiple transactions by a user without these being linkable to each other
Transactions can be made with an unlimited number of service providers with a single credential\\
\bottomrule
\end{tabular}
\end{table*}

==> questionnaire.tex <==
\clearpage
\onecolumn
\begin{longtable}[c]{llp{9cm}l}
\caption{Adapted questionnaires on perceived trustworthiness and technology acceptance of \ACS.
All questions are 7-point Likert items, anchored on 1=\emph{Strongly Disagree} to 7=\emph{Strongly Agree}.
(\textbf{R}) marks reverse-coded items. Questions modified from their original format show the modifications in \textbf{bold}.}\\
  \toprule
Construct & Item & Format & Source  \\ 
  \midrule
\endfirsthead
  \toprule
Construct & Item & Format & Source  \\ 
  \midrule
 \endhead
 \bottomrule
   \endfoot
 \bottomrule
 \endlastfoot
 \multicolumn{4}{l}{\emph{Faith in General Technology}~\cite{mcknight2011trust}: Unmodified}\\
 \addlinespace
\multirow{4}{*}{Faith in Technology (\textsf{fit})} & \textsf{MKF1} & I believe that most technologies are effective at what they are designed to do. & \cite{mcknight2011trust}\\
 & \textsf{MKF2} & A large majority of technologies are excellent. & \cite{mcknight2011trust}\\
 & \textsf{MKF3} & Most technologies have the features needed for their domain. & \cite{mcknight2011trust}\\
 & \textsf{MKF4} & I think most technologies enable me to do what I need to do. & \cite{mcknight2011trust}\\
\addlinespace
 \multirow{3}{*}{Trusting Stance (\textsf{ts})} & \textsf{MKTS1} & My typical approach is to trust new technologies until they prove to me that I shouldn't trust them. & \cite{mcknight2011trust}\\
 & \textsf{MKTS2} & I usually trust a technology until it gives me a reason not to trust it. & \cite{mcknight2011trust}\\
 & \textsf{MKTS3} & I generally give a technology the benefit of the doubt when I first use it. & \cite{mcknight2011trust}\\
\midrule
 \multicolumn{4}{l}{\emph{Internet users' information privacy concerns (IUIPC)}~\cite{malhotra2004internet}: Unmodified}\\
 \addlinespace
\multirow{3}{*}{Control (\textsf{ctrl})} & \textsf{ctrl1} & Consumer online privacy is really a matter of consumers' right to exercise control and autonomy over decisions about how their information is collected, used, and shared.  & \cite{malhotra2004internet}\\
 & \textsf{ctrl2} & Consumer control of personal information lies at the heart of consumer privacy.  &  \cite{malhotra2004internet}\\
 & \textsf{ctrl3} & I believe that online privacy is invaded when control is lost or unwillingly reduced as a result of a marketing transaction.  &  \cite{malhotra2004internet}\\
\addlinespace
 \multirow{3}{*}{Awareness (\textsf{aware})} & \textsf{awa1} & Companies seeking information online should disclose the way the data are collected, processed, and used.  & \cite{malhotra2004internet}\\
 & \textsf{awa2} & A good consumer online privacy policy should have a clear and conspicuous disclosure. & \cite{malhotra2004internet}\\
 & \textsf{awa3} & It is very important to me that I am aware and knowledgeable about how my personal information will be used.  & \cite{malhotra2004internet}\\
 \addlinespace
 \multirow{4}{*}{Collection (\textsf{collect})} & \textsf{coll1} & It usually bothers me when online companies ask me for personal information.   & \cite{malhotra2004internet}\\
 & \textsf{coll2} & When online companies ask me for personal information, I sometimes think twice before providing it.  & \cite{malhotra2004internet}\\
 & \textsf{coll3} & It bothers me to give personal information to so many online companies.   & \cite{malhotra2004internet}\\
 & \textsf{coll4} & I'm concerned that online companies are collecting too much personal information about me.   & \cite{malhotra2004internet}\\
\midrule
\multicolumn{4}{l}{\emph{System Trustworthiness \& Acceptance}~\cite{alalwan2017factors}: Refer to ``\ACS'' as object and ``privacy'' as secondary property.}\\
 \addlinespace
\multirow{4}{*}{\begin{minipage}{4.5cm}Performance Expectancy (\textsf{perfexp})\\
$\Longleftrightarrow$ Primary Usefulness (\textsf{primuse})\end{minipage}} & \textsf{STPE1} & I \textbf{would} find \textbf{anonymous credential systems} useful in my daily life. & \cite{alalwan2017factors}\\
 & \textsf{STPE2} & Using \textbf{anonymous credential systems} increases my chances of achieving tasks that are important to me. &  \cite{alalwan2017factors}\\
  & \textsf{STPE3} & Using \textbf{anonymous credential systems} helps me accomplish tasks more quickly. &  \cite{alalwan2017factors}\\
  & \textsf{STPE4} & Using \textbf{anonymous credential systems} increases my productivity. &  \cite{alalwan2017factors}\\
\addlinespace
\multirow{4}{*}{\begin{minipage}{4.5cm}Effort Expectancy (\textsf{effexp})\\
$\Longleftrightarrow$ Ease of Use (\textsf{ease})\end{minipage}} & \textsf{STEE1} & Learning how to use \textbf{anonymous credential systems} is easy for me.  & \cite{alalwan2017factors}\\
 & \textsf{STEE2} & My interaction with \textbf{anonymous credential systems} is clear and understandable. &  \cite{alalwan2017factors}\\
  & \textsf{STEE3} & I find \textbf{anonymous credential systems} easy to use. &  \cite{alalwan2017factors}\\
  & \textsf{STEE4} & It is easy for me to become skilful at using \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
\addlinespace
\multirow{3}{*}{Social Influence (\textsf{si})} & \textsf{STSI1} & People who are important to me think that I should use \textbf{a system, such as an anonymous credential system, to protect my privacy}. & \cite{alalwan2017factors}\\
 & \textsf{STSI2} & People who influence my behaviour think that I should use \textbf{a system, such as an anonymous credential system, to protect my privacy}. &  \cite{alalwan2017factors}\\
  & \textsf{STSI3} & People whose opinions that I value prefer that I use \textbf{a system, such as an anonymous credential system, to protect my privacy}. &  \cite{alalwan2017factors}\\
\addlinespace
\multirow{4}{*}{Facilitating Conditions (\textsf{fc})} & \textsf{STFC1} & I have the resources necessary to use \textbf{anonymous credential systems}.  & \cite{alalwan2017factors}\\
 & \textsf{STFC2} & I have the knowledge necessary to use \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
  & \textsf{STFC3} & \textbf{Anonymous credential systems are} compatible with other technologies I use. &  \cite{alalwan2017factors}\\
  & \textsf{STFC4} & I can get help from others when I have difficulties using \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
\addlinespace
\multirow{4}{*}{Behvarioral Intention (\textsf{bi})} & \textsf{STBI1} & I intend to use \textbf{anonymous credential systems} in the future.  & \cite{alalwan2017factors}\\
 & \textsf{STBI2} & I will always try to use \textbf{anonymous credential systems} in my daily life. &  \cite{alalwan2017factors}\\
  & \textsf{STBI3} & I plan to use \textbf{anonymous credential systems} in future. &  \cite{alalwan2017factors}\\
  & \textsf{STBI4} & I predict I would use \textbf{anonymous credential systems} in the future. &  \cite{alalwan2017factors}\\
\addlinespace
\multirow{6}{*}{Perceived Trustworthiness (\textsf{trust})} & \textsf{STT1} & I believe that \textbf{anonymous credential systems} are trustworthy. & \cite{alalwan2017factors}\\
 & \textsf{STT2} & I trust in \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
  & \textsf{STT3} & I do not doubt the honesty of \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
  & \textsf{STT4} & I feel assured that legal and technological structures adequately protect me from problems on \textbf{anonymous credential systems}. &  \cite{alalwan2017factors}\\
    & \textsf{STT5} & Even if not monitored, I would trust \textbf{anonymous credential systems} to do the job right. &  \cite{alalwan2017factors}\\
  & \textsf{STT6} & \textbf{Anonymous credential systems} have the ability to fulfil their task. &  \cite{alalwan2017factors}\\
\midrule
\multicolumn{4}{l}{\emph{Technology Acceptance Model (TAM 2.0)}~\cite{venkatesh2000theoretical}: Refer to ``\ACS'' as object and ``privacy'' as secondary property.}\\
 \addlinespace
\multirow{4}{*}{\begin{minipage}{4.5cm}Perceived Usefulness (\textsf{useful})\\
$\Longleftrightarrow$ Secondary Usefulness \\
$\Longleftrightarrow$ Privacy Usefulness (\textsf{privuse})\end{minipage}} & \textsf{TAU1} & Using the system improves my \textbf{ability to do what I need to in terms of privacy protection}. & \cite{venkatesh2000theoretical}\\
 & \textsf{TAU2} & Using the system in my \textbf{day to day life increases my privacy protection}. &  \cite{venkatesh2000theoretical}\\
  & \textsf{TAU3} & Using the system enhances the \textbf{privacy of my personal information}. &  \cite{venkatesh2000theoretical}\\
  & \textsf{TAU4} & I find the system to useful to \textbf{complete tasks requiring privacy protection}. &  \cite{venkatesh2000theoretical}\\
\addlinespace
\multirow{4}{*}{\begin{minipage}{4.5cm}Perceived Ease of Use (\textsf{ease})\end{minipage}} & \textsf{TAE1} & My interaction with the system is clear and understandable. & \cite{venkatesh2000theoretical}\\
 & \textsf{TAE2} & Interacting with the system does not require a lot of my mental effort. &  \cite{venkatesh2000theoretical}\\
  & \textsf{TAE3} & I find it easy to get the system to do what I want it to do. &  \cite{venkatesh2000theoretical}\\
  & \textsf{TAE4} & I find the system to be easy to use. &  \cite{venkatesh2000theoretical}\\
\addlinespace
\multirow{4}{*}{Results Demonstrability (\textsf{results})} & \textsf{TAR1} & I have no difficulty telling others about the results of using the system. & \cite{venkatesh2000theoretical}\\
 & \textsf{TAR2} & I believe I could communicate to others the consequences of using the system. &  \cite{venkatesh2000theoretical}\\
  & \textsf{TAR3} & The results of using the system are apparent to me. &  \cite{venkatesh2000theoretical}\\
  & \sout{\textsf{rTAR4}} & \sout{I would have difficulty explaining why using the system may or may not be beneficial.} (\textbf{R}) [\emph{Removed due to inconsistency with sub-scale.}] &  \cite{venkatesh2000theoretical}\\
\midrule
 \multicolumn{4}{l}{\emph{\textbf{Not included in the final model}}}\\
\midrule
 \multicolumn{4}{l}{\emph{Trustworthiness Provider}~\cite{buttner2008perceived}: Refer to subject as ``user''}\\
 \addlinespace
\multirow{3}{*}{Ability (\textsf{ability})} & \textsf{TPA1} & This provider is very competent. & \cite{buttner2008perceived}\\
 & \textsf{TPA2} & This provider is able to fully satisfy its \textbf{users}. & \cite{buttner2008perceived}\\
 & \textsf{TPA3} & One can expect good advice from this provider. & \cite{buttner2008perceived}\\
\addlinespace
\multirow{3}{*}{Benevolence (\textsf{benevol})} & \textsf{TPB1} & This provider is genuinely interested in its \textbf{users'} welfare. & \cite{buttner2008perceived}\\
 & \textsf{TPB2} & This provider puts \textbf{users'} interests first. & \cite{buttner2008perceived}\\
 & \textsf{TPB3} & If problems arise, one can expect to be treated fairly by this provider. & \cite{buttner2008perceived}\\
 \addlinespace
\multirow{3}{*}{Integrity (\textsf{integrity})} & \textsf{TPI1} & I am happy with the standards by which this provider is operating. & \cite{buttner2008perceived}\\
 & \textsf{TPI2} & This provider operates scrupulously. & \cite{buttner2008perceived}\\
 & \textsf{TPI3} & You can believe the statements of this provider. & \cite{buttner2008perceived}\\
  \addlinespace
\multirow{3}{*}{Predictability (\textsf{predict})} & \textsf{r}\textsf{TPP1} & This provider's methods of operation are unclear. (\textbf{R}) & \cite{buttner2008perceived}\\
 & \textsf{TPP2} & This provider keeps its promises. & \cite{buttner2008perceived}\\
 & \textsf{TPP3} & I would rely on advice from this provider. & \cite{buttner2008perceived}\\
\midrule
\multicolumn{4}{l}{\emph{Alternative System Trustworthiness}~\cite{corritore2005measuring}: Refer to object ``Website'' as \ACS}\\
 \addlinespace
\multirow{3}{*}{Honesty (\textsf{honest})} & \textsf{STCH1} & The \textbf{anonymous credential system} provides truthful information. & \cite{corritore2005measuring}\\
 & \textsf{STCH2} & The \textbf{anonymous credential system} is believable. & \cite{corritore2005measuring}\\
 & \textsf{STCH3} & The features of the \textbf{anonymous credential system} reflect expertise. & \cite{corritore2005measuring}\\
  \addlinespace
\multirow{2}{*}{Reputation (\textsf{rep})} & \textsf{STCRe1} & The \textbf{anonymous credential system} is respected. & \cite{corritore2005measuring}\\
 & \textsf{STCRe2} & The \textbf{anonymous credential system} has a good reputation. & \cite{corritore2005measuring}\\
\addlinespace
\multirow{4}{*}{Risk (\textsf{risk})} & \textsf{STCR1} & I am taking a chance interacting with this \textbf{anonymous credential system}. & \cite{corritore2005measuring}\\
 & \textsf{STCR2} & I feel that it is unsafe to interact with this \textbf{anonymous credential system}. & \cite{corritore2005measuring}\\
 & \textsf{STCR3} & I feel I must be cautious when using this \textbf{anonymous credential system}. & \cite{corritore2005measuring}\\
 & \textsf{STCR4} & It is risky to interact with this \textbf{anonymous credential system}. & \cite{corritore2005measuring}\\
\midrule
\multicolumn{4}{l}{\emph{Trusting Belief Reliability}~\cite{mcknight2011trust}: Refer to object \ACS}\\
 \addlinespace
\multirow{3}{*}{Reliability (\textsf{reliable})} & \textsf{TB1} & The \textbf{anonymous credential system} is a very reliable piece of software. & \cite{mcknight2011trust}\\
 & \textsf{TB2} & The \textbf{anonymous credential system} does not fail me. & \cite{mcknight2011trust}\\
 & \textsf{TB3} & The \textbf{anonymous credential system} is extremely dependable. & \cite{mcknight2011trust}\\
 & \textsf{TB4} & The \textbf{anonymous credential system} does not malfunction for me. & \cite{mcknight2011trust}\\
\end{longtable}
 \clearpage
\twocolumn

==> residual_correlations.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Feb 27 19:31:58 2020
\begin{table*}[ht]
\centering
\caption{Residual Correlations.} 
\label{tab:residualsCov}
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
  \toprule
 & IUIPC1 & IUIPC2 & IUIPC3 & IUIPC4 & IUIPC5 & IUIPC6 & IUIPC7 & IUIPC8 & IUIPC9 & IUIPC10 & MKF1 & MKF2 & MKF3 & MKF4 & MKTS1 & MKTS2 & MKTS3 & STSI1 & STSI2 & STSI3 & TAR1 & TAR2 & TAR3 & STFC1 & STFC2 & STFC3 & STFC4 & STT1 & STT2 & STT3 & STT4 & STT5 & STT6 & STPE1 & STPE2 & STPE3 & STPE4 & TAU1 & TAU2 & TAU3 & TAU4 & TAE1 & TAE2 & TAE3 & TAE4 & STBI1 & STBI2 & STBI3 & STBI4 & d\_gov & d\_company & d\_university & benefits & usage & simplicity & people & d\_fullsupport & d\_contact \\ 
  \midrule
IUIPC1 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC2 & -0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC3 & -0.00 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC4 & 0.01 & 0.03 & -0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC5 & 0.00 & 0.01 & -0.03 & 0.02 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC6 & 0.04 & 0.05 & 0.03 & -0.04 & -0.02 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC7 & -0.13 & -0.10 & 0.03 & -0.12 & -0.07 & 0.16 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC8 & -0.02 & -0.03 & 0.09 & 0.00 & 0.04 & 0.20 & 0.04 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC9 & -0.06 & -0.10 & 0.04 & -0.07 & -0.03 & 0.21 & 0.00 & -0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  IUIPC10 & -0.04 & -0.05 & 0.07 & 0.03 & 0.02 & 0.24 & -0.01 & -0.03 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKF1 & 0.10 & 0.01 & -0.04 & -0.05 & -0.03 & 0.04 & -0.04 & 0.01 & 0.01 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKF2 & 0.10 & 0.04 & -0.05 & 0.02 & -0.02 & 0.04 & -0.04 & 0.00 & -0.00 & 0.00 & 0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKF3 & 0.09 & 0.05 & -0.03 & 0.00 & -0.02 & 0.00 & -0.02 & 0.01 & 0.03 & -0.01 & 0.00 & 0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKF4 & 0.09 & 0.07 & -0.08 & 0.02 & 0.03 & 0.07 & -0.05 & 0.01 & -0.01 & -0.01 & -0.01 & -0.02 & -0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKTS1 & 0.11 & 0.06 & -0.08 & -0.03 & -0.01 & -0.00 & -0.02 & -0.01 & 0.00 & -0.00 & -0.01 & -0.01 & -0.04 & 0.06 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKTS2 & 0.12 & 0.08 & -0.06 & 0.00 & 0.01 & 0.01 & -0.01 & 0.00 & -0.00 & 0.03 & -0.01 & -0.02 & -0.02 & 0.06 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  MKTS3 & 0.07 & 0.05 & 0.00 & 0.02 & 0.02 & 0.03 & -0.02 & 0.01 & 0.02 & 0.01 & 0.02 & 0.01 & 0.01 & 0.10 & -0.00 & -0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STSI1 & 0.06 & 0.03 & -0.04 & -0.02 & -0.03 & 0.15 & -0.01 & 0.03 & 0.01 & 0.00 & 0.01 & -0.01 & 0.03 & -0.01 & 0.01 & 0.01 & 0.07 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STSI2 & 0.04 & 0.01 & -0.02 & -0.01 & -0.03 & 0.17 & -0.02 & -0.02 & -0.00 & 0.01 & -0.01 & -0.01 & 0.01 & -0.01 & -0.01 & 0.00 & 0.04 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STSI3 & 0.02 & -0.00 & -0.02 & -0.04 & -0.05 & 0.15 & -0.01 & -0.01 & -0.00 & 0.01 & 0.00 & -0.00 & 0.02 & -0.02 & -0.03 & -0.01 & 0.05 & -0.00 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAR1 & 0.04 & 0.04 & -0.04 & -0.02 & -0.00 & 0.10 & -0.01 & 0.02 & 0.04 & 0.05 & -0.01 & -0.03 & 0.02 & 0.01 & -0.02 & -0.00 & 0.05 & 0.04 & 0.03 & 0.02 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAR2 & 0.07 & 0.07 & -0.03 & 0.00 & -0.02 & 0.05 & -0.05 & -0.01 & -0.02 & -0.00 & -0.02 & -0.00 & -0.01 & -0.00 & -0.05 & -0.03 & 0.02 & -0.04 & -0.03 & -0.03 & 0.02 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAR3 & 0.05 & 0.05 & -0.04 & -0.00 & -0.02 & 0.02 & -0.06 & 0.00 & -0.01 & -0.01 & -0.02 & 0.03 & 0.01 & 0.01 & -0.01 & 0.02 & 0.06 & 0.01 & -0.00 & -0.01 & -0.05 & 0.04 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STFC1 & 0.02 & 0.06 & 0.01 & 0.06 & -0.01 & 0.04 & 0.01 & 0.06 & 0.05 & 0.03 & -0.07 & -0.07 & -0.02 & 0.02 & -0.09 & -0.05 & 0.02 & -0.04 & -0.01 & -0.01 & -0.02 & 0.00 & -0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STFC2 & 0.03 & 0.06 & 0.00 & -0.02 & -0.02 & 0.05 & -0.03 & 0.06 & 0.02 & 0.02 & -0.06 & -0.04 & -0.02 & -0.04 & -0.04 & -0.05 & 0.05 & -0.00 & -0.00 & 0.01 & 0.01 & 0.04 & 0.04 & -0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STFC3 & 0.05 & 0.07 & -0.05 & -0.01 & -0.02 & 0.02 & -0.04 & 0.01 & 0.02 & -0.01 & 0.01 & 0.03 & 0.02 & 0.06 & -0.01 & 0.01 & 0.04 & -0.01 & -0.00 & 0.01 & -0.00 & -0.06 & -0.04 & 0.04 & -0.01 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STFC4 & 0.04 & 0.07 & -0.08 & -0.01 & 0.01 & 0.07 & -0.07 & -0.03 & -0.03 & -0.01 & 0.02 & 0.01 & 0.03 & 0.05 & 0.05 & 0.04 & 0.08 & 0.04 & 0.02 & 0.02 & 0.04 & -0.01 & -0.00 & -0.03 & -0.06 & 0.06 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT1 & 0.12 & 0.11 & 0.01 & 0.09 & 0.05 & 0.09 & -0.13 & -0.09 & -0.05 & -0.08 & 0.27 & 0.26 & 0.27 & 0.20 & 0.24 & 0.28 & 0.23 & 0.40 & 0.41 & 0.40 & 0.48 & 0.33 & 0.48 & 0.31 & 0.37 & 0.46 & 0.41 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT2 & 0.13 & 0.14 & -0.01 & 0.06 & 0.03 & 0.05 & -0.15 & -0.09 & -0.09 & -0.11 & 0.28 & 0.27 & 0.26 & 0.23 & 0.28 & 0.30 & 0.27 & 0.39 & 0.40 & 0.39 & 0.47 & 0.33 & 0.47 & 0.33 & 0.39 & 0.47 & 0.42 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT3 & 0.05 & 0.08 & -0.06 & 0.01 & 0.02 & 0.05 & -0.13 & -0.11 & -0.07 & -0.09 & 0.25 & 0.28 & 0.26 & 0.20 & 0.32 & 0.34 & 0.30 & 0.32 & 0.31 & 0.30 & 0.38 & 0.30 & 0.43 & 0.23 & 0.29 & 0.37 & 0.37 & -0.02 & 0.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT4 & 0.12 & 0.12 & -0.04 & 0.03 & 0.02 & 0.13 & -0.12 & -0.12 & -0.09 & -0.10 & 0.30 & 0.30 & 0.26 & 0.25 & 0.32 & 0.35 & 0.29 & 0.34 & 0.34 & 0.36 & 0.45 & 0.33 & 0.48 & 0.27 & 0.36 & 0.43 & 0.42 & -0.02 & -0.02 & 0.05 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT5 & 0.04 & 0.03 & -0.07 & -0.08 & -0.09 & -0.01 & -0.09 & -0.14 & -0.08 & -0.08 & 0.21 & 0.23 & 0.20 & 0.15 & 0.29 & 0.31 & 0.28 & 0.29 & 0.30 & 0.31 & 0.32 & 0.22 & 0.31 & 0.17 & 0.27 & 0.29 & 0.29 & -0.03 & -0.02 & 0.03 & 0.05 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STT6 & 0.12 & 0.16 & 0.06 & 0.12 & 0.10 & 0.03 & -0.12 & -0.02 & -0.06 & -0.07 & 0.23 & 0.25 & 0.27 & 0.21 & 0.21 & 0.22 & 0.23 & 0.29 & 0.30 & 0.29 & 0.48 & 0.40 & 0.51 & 0.33 & 0.38 & 0.47 & 0.41 & 0.03 & 0.03 & -0.04 & -0.02 & -0.03 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STPE1 & 0.10 & 0.05 & 0.09 & 0.16 & 0.12 & 0.14 & 0.07 & 0.09 & 0.10 & 0.12 & 0.08 & 0.08 & 0.11 & 0.09 & 0.06 & 0.07 & 0.11 & 0.13 & 0.08 & 0.09 & 0.19 & 0.13 & 0.18 & 0.11 & 0.12 & 0.17 & 0.15 & 0.31 & 0.27 & 0.13 & 0.16 & 0.06 & 0.28 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STPE2 & 0.07 & 0.02 & 0.04 & 0.06 & 0.02 & 0.15 & 0.04 & 0.05 & 0.07 & 0.09 & 0.06 & 0.06 & 0.10 & 0.03 & 0.09 & 0.10 & 0.10 & 0.13 & 0.11 & 0.13 & 0.13 & 0.06 & 0.11 & 0.07 & 0.10 & 0.13 & 0.14 & 0.25 & 0.21 & 0.10 & 0.15 & 0.14 & 0.19 & 0.10 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STPE3 & 0.02 & -0.02 & 0.04 & 0.05 & -0.01 & 0.10 & -0.02 & 0.00 & -0.00 & 0.02 & 0.08 & 0.08 & 0.06 & 0.06 & 0.08 & 0.09 & 0.10 & 0.06 & 0.01 & 0.03 & 0.09 & 0.02 & 0.10 & 0.08 & 0.09 & 0.08 & 0.10 & 0.19 & 0.16 & 0.07 & 0.12 & 0.07 & 0.17 & -0.04 & 0.04 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STPE4 & 0.01 & -0.03 & 0.02 & 0.03 & -0.01 & 0.12 & -0.01 & -0.01 & 0.00 & 0.03 & 0.07 & 0.08 & 0.09 & 0.04 & 0.08 & 0.09 & 0.10 & 0.10 & 0.05 & 0.08 & 0.09 & 0.01 & 0.08 & 0.06 & 0.10 & 0.10 & 0.14 & 0.24 & 0.20 & 0.10 & 0.17 & 0.12 & 0.17 & -0.02 & -0.02 & 0.10 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAU1 & 0.07 & 0.07 & 0.00 & 0.04 & 0.00 & 0.04 & -0.08 & 0.01 & -0.02 & 0.00 & 0.10 & 0.11 & 0.13 & 0.08 & 0.13 & 0.14 & 0.14 & 0.18 & 0.19 & 0.17 & 0.16 & 0.09 & 0.18 & 0.10 & 0.10 & 0.18 & 0.16 & 0.21 & 0.16 & 0.06 & 0.09 & -0.02 & 0.23 & 0.34 & 0.20 & 0.16 & 0.15 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAU2 & 0.06 & 0.06 & -0.04 & 0.01 & -0.03 & -0.03 & -0.14 & -0.05 & -0.07 & -0.05 & 0.10 & 0.13 & 0.13 & 0.11 & 0.13 & 0.13 & 0.12 & 0.17 & 0.18 & 0.17 & 0.16 & 0.09 & 0.18 & 0.10 & 0.11 & 0.20 & 0.15 & 0.20 & 0.16 & 0.07 & 0.09 & 0.01 & 0.24 & 0.33 & 0.18 & 0.16 & 0.16 & 0.04 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAU3 & 0.03 & 0.02 & -0.05 & 0.01 & 0.00 & -0.02 & -0.15 & -0.06 & -0.09 & -0.06 & 0.10 & 0.11 & 0.12 & 0.13 & 0.15 & 0.14 & 0.14 & 0.16 & 0.15 & 0.15 & 0.15 & 0.07 & 0.17 & 0.09 & 0.07 & 0.19 & 0.14 & 0.21 & 0.18 & 0.08 & 0.09 & -0.00 & 0.22 & 0.30 & 0.15 & 0.12 & 0.12 & 0.04 & 0.02 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAU4 & 0.02 & 0.02 & -0.03 & 0.02 & -0.00 & 0.01 & -0.09 & -0.02 & -0.03 & -0.01 & 0.12 & 0.12 & 0.13 & 0.10 & 0.16 & 0.16 & 0.13 & 0.22 & 0.21 & 0.21 & 0.20 & 0.11 & 0.21 & 0.10 & 0.12 & 0.17 & 0.18 & 0.23 & 0.21 & 0.09 & 0.09 & 0.03 & 0.24 & 0.35 & 0.23 & 0.20 & 0.20 & 0.02 & 0.03 & 0.05 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAE1 & 0.03 & 0.03 & -0.02 & -0.03 & -0.02 & 0.11 & -0.03 & 0.01 & -0.02 & -0.01 & 0.03 & 0.07 & 0.05 & 0.04 & 0.05 & 0.05 & 0.09 & 0.07 & 0.06 & 0.06 & 0.08 & -0.03 & 0.13 & 0.05 & 0.10 & 0.01 & 0.06 & 0.42 & 0.38 & 0.31 & 0.40 & 0.29 & 0.38 & 0.21 & 0.16 & 0.17 & 0.16 & 0.21 & 0.18 & 0.19 & 0.26 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAE2 & 0.02 & 0.04 & 0.03 & 0.06 & 0.01 & 0.05 & -0.05 & -0.01 & -0.05 & -0.01 & 0.02 & 0.07 & 0.05 & 0.08 & -0.00 & 0.02 & 0.03 & -0.06 & -0.06 & -0.06 & 0.05 & -0.01 & 0.06 & 0.07 & 0.12 & -0.03 & -0.03 & 0.27 & 0.25 & 0.16 & 0.22 & 0.17 & 0.32 & 0.12 & 0.04 & 0.09 & 0.07 & 0.09 & 0.09 & 0.10 & 0.16 & 0.06 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAE3 & 0.01 & 0.02 & -0.04 & -0.01 & -0.04 & 0.05 & -0.08 & -0.03 & -0.04 & -0.03 & 0.04 & 0.06 & 0.08 & 0.06 & 0.06 & 0.07 & 0.11 & 0.01 & 0.03 & 0.03 & 0.08 & -0.05 & 0.03 & 0.02 & 0.07 & 0.01 & 0.02 & 0.34 & 0.33 & 0.24 & 0.31 & 0.24 & 0.37 & 0.10 & 0.06 & 0.10 & 0.10 & 0.12 & 0.15 & 0.15 & 0.20 & 0.03 & 0.05 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  TAE4 & 0.01 & 0.01 & -0.04 & -0.00 & -0.03 & 0.09 & -0.04 & -0.02 & -0.01 & -0.01 & 0.03 & 0.05 & 0.06 & 0.03 & 0.07 & 0.08 & 0.08 & 0.01 & 0.03 & 0.02 & 0.12 & 0.01 & 0.05 & 0.06 & 0.10 & 0.01 & 0.04 & 0.30 & 0.28 & 0.24 & 0.29 & 0.24 & 0.34 & 0.07 & 0.04 & 0.04 & 0.05 & 0.10 & 0.07 & 0.08 & 0.15 & 0.00 & 0.05 & 0.07 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STBI1 & 0.06 & 0.04 & 0.02 & 0.07 & 0.01 & 0.12 & 0.06 & 0.05 & 0.07 & 0.09 & 0.01 & 0.04 & 0.05 & 0.03 & 0.06 & 0.08 & 0.10 & 0.19 & 0.18 & 0.20 & 0.14 & 0.08 & 0.11 & 0.10 & 0.14 & 0.22 & 0.20 & 0.33 & 0.30 & 0.17 & 0.21 & 0.16 & 0.27 & 0.22 & 0.08 & -0.02 & -0.00 & 0.12 & 0.09 & 0.07 & 0.16 & 0.13 & 0.06 & 0.04 & 0.03 &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STBI2 & 0.09 & 0.04 & 0.01 & 0.05 & -0.00 & 0.14 & 0.07 & 0.03 & 0.09 & 0.11 & 0.03 & 0.11 & 0.09 & 0.04 & 0.10 & 0.11 & 0.12 & 0.25 & 0.24 & 0.26 & 0.18 & 0.11 & 0.15 & 0.11 & 0.15 & 0.21 & 0.20 & 0.36 & 0.34 & 0.20 & 0.26 & 0.23 & 0.27 & 0.24 & 0.18 & 0.07 & 0.09 & 0.14 & 0.12 & 0.09 & 0.16 & 0.19 & 0.08 & 0.09 & 0.08 & 0.03 &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  STBI3 & 0.07 & 0.03 & 0.02 & 0.07 & 0.02 & 0.12 & 0.05 & 0.06 & 0.08 & 0.09 & 0.02 & 0.04 & 0.03 & 0.05 & 0.07 & 0.07 & 0.10 & 0.19 & 0.17 & 0.18 & 0.16 & 0.10 & 0.15 & 0.10 & 0.15 & 0.18 & 0.17 & 0.33 & 0.31 & 0.15 & 0.19 & 0.16 & 0.28 & 0.24 & 0.08 & -0.00 & 0.01 & 0.14 & 0.11 & 0.09 & 0.18 & 0.13 & 0.07 & 0.05 & 0.03 & 0.02 & 0.02 &  &  &  &  &  &  &  &  &  &  &  \\ 
  STBI4 & 0.07 & 0.04 & 0.01 & 0.06 & 0.01 & 0.11 & 0.02 & 0.05 & 0.06 & 0.06 & 0.03 & 0.03 & 0.05 & 0.04 & 0.05 & 0.06 & 0.08 & 0.18 & 0.16 & 0.17 & 0.14 & 0.08 & 0.14 & 0.09 & 0.11 & 0.20 & 0.18 & 0.34 & 0.32 & 0.17 & 0.19 & 0.13 & 0.29 & 0.28 & 0.10 & 0.01 & 0.01 & 0.17 & 0.14 & 0.12 & 0.20 & 0.14 & 0.08 & 0.05 & 0.03 & 0.03 & 0.01 & 0.02 &  &  &  &  &  &  &  &  &  &  \\ 
  d\_gov & 0.02 & 0.02 & 0.03 & 0.02 & 0.01 & 0.05 & 0.04 & 0.01 & 0.04 & 0.04 & 0.02 & 0.00 & 0.05 & -0.01 & 0.00 & 0.01 & -0.02 & -0.04 & -0.02 & -0.01 & 0.02 & 0.01 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & -0.00 & -0.01 & 0.01 & -0.01 & -0.01 & 0.04 & -0.08 & -0.02 & 0.04 & -0.00 & 0.01 & 0.02 & 0.01 & 0.03 & 0.02 & 0.05 & 0.01 & 0.02 & -0.01 & -0.01 & -0.05 & -0.03 &  &  &  &  &  &  &  &  &  \\ 
  d\_company & 0.02 & 0.02 & 0.00 & 0.05 & 0.01 & 0.04 & 0.00 & 0.03 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.01 & 0.04 & 0.01 & -0.00 & 0.03 & 0.04 & 0.00 & 0.07 & 0.10 & 0.08 & 0.04 & 0.04 & -0.02 & 0.02 & -0.02 & -0.02 & 0.01 & -0.00 & 0.01 & 0.03 & -0.03 & 0.00 & 0.07 & 0.03 & 0.03 & 0.04 & 0.03 & 0.05 & 0.04 & 0.07 & 0.04 & 0.04 & -0.02 & -0.01 & -0.01 & 0.00 & 0.00 &  &  &  &  &  &  &  &  \\ 
  d\_university & 0.00 & 0.01 & 0.03 & 0.03 & 0.04 & -0.03 & -0.04 & -0.05 & -0.06 & -0.07 & -0.03 & 0.02 & -0.04 & -0.03 & -0.02 & -0.02 & -0.07 & 0.01 & 0.03 & 0.02 & 0.01 & 0.03 & 0.05 & 0.04 & 0.05 & 0.01 & -0.01 & 0.03 & 0.02 & 0.02 & -0.03 & -0.07 & 0.02 & 0.03 & -0.01 & 0.02 & 0.02 & 0.02 & 0.00 & 0.00 & 0.01 & 0.05 & 0.04 & 0.02 & -0.02 & 0.00 & -0.00 & -0.00 & 0.01 & 0.00 & 0.00 &  &  &  &  &  &  &  \\ 
  benefits & -0.02 & -0.00 & -0.01 & -0.03 & -0.01 & -0.01 & 0.04 & 0.03 & 0.01 & 0.01 & 0.04 & 0.02 & 0.01 & 0.04 & -0.00 & 0.03 & 0.07 & -0.03 & -0.06 & -0.04 & -0.01 & -0.05 & -0.09 & -0.06 & -0.07 & -0.03 & -0.00 & -0.03 & 0.00 & -0.01 & 0.01 & 0.03 & 0.00 & 0.01 & 0.01 & -0.07 & -0.05 & -0.02 & -0.03 & -0.01 & -0.03 & -0.08 & -0.06 & -0.01 & -0.00 & 0.02 & 0.01 & 0.05 & -0.00 & 0.00 & 0.00 & 0.00 &  &  &  &  &  &  \\ 
  usage & -0.05 & -0.06 & -0.08 & -0.08 & -0.05 & -0.01 & -0.00 & 0.00 & -0.01 & 0.01 & 0.00 & -0.02 & -0.02 & -0.01 & -0.01 & -0.00 & 0.03 & -0.06 & -0.08 & -0.06 & -0.02 & -0.05 & -0.08 & -0.08 & -0.09 & -0.08 & 0.02 & -0.01 & 0.02 & 0.00 & 0.01 & 0.02 & -0.08 & 0.02 & 0.01 & -0.08 & -0.05 & -0.04 & -0.03 & -0.01 & -0.05 & -0.06 & -0.08 & -0.03 & -0.02 & 0.02 & 0.01 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  &  &  &  &  \\ 
  simplicity & -0.01 & -0.00 & 0.04 & 0.04 & 0.07 & 0.05 & -0.00 & -0.03 & -0.02 & 0.00 & 0.01 & 0.02 & 0.02 & -0.00 & -0.01 & -0.02 & -0.04 & 0.02 & 0.05 & 0.05 & 0.14 & 0.15 & 0.18 & 0.17 & 0.17 & 0.06 & 0.09 & -0.01 & -0.01 & -0.02 & 0.01 & -0.02 & 0.06 & 0.02 & 0.01 & 0.09 & 0.05 & 0.07 & 0.06 & 0.03 & 0.11 & 0.14 & 0.13 & 0.07 & 0.08 & 0.03 & 0.06 & 0.02 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  &  &  &  \\ 
  people & 0.05 & 0.05 & 0.02 & 0.10 & 0.08 & 0.08 & 0.01 & 0.03 & 0.01 & 0.01 & -0.00 & 0.03 & -0.01 & 0.03 & -0.01 & -0.03 & -0.06 & -0.01 & 0.01 & 0.02 & 0.04 & 0.10 & 0.10 & 0.09 & 0.10 & 0.04 & 0.01 & 0.01 & 0.01 & -0.02 & -0.02 & -0.05 & 0.07 & -0.02 & -0.01 & 0.07 & 0.04 & 0.06 & 0.06 & 0.04 & 0.03 & 0.06 & 0.12 & 0.05 & 0.02 & -0.02 & -0.01 & -0.01 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  &  &  \\ 
  d\_fullsupport & -0.04 & -0.06 & -0.05 & -0.02 & -0.01 & 0.03 & 0.04 & -0.02 & 0.00 & -0.01 & -0.03 & -0.03 & -0.02 & -0.00 & -0.00 & -0.01 & -0.05 & -0.03 & -0.05 & -0.02 & -0.05 & -0.04 & -0.06 & -0.08 & -0.08 & -0.01 & -0.03 & 0.02 & 0.01 & -0.02 & 0.01 & 0.01 & -0.04 & -0.00 & -0.01 & -0.05 & 0.00 & -0.04 & -0.02 & 0.00 & -0.03 & -0.06 & -0.08 & -0.02 & -0.00 & -0.00 & 0.01 & 0.01 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  &  \\ 
  d\_contact & -0.06 & -0.01 & -0.06 & -0.10 & -0.07 & -0.04 & -0.03 & 0.02 & 0.00 & -0.00 & 0.02 & -0.02 & -0.03 & 0.01 & 0.00 & 0.02 & 0.06 & 0.01 & 0.01 & 0.01 & 0.04 & 0.02 & 0.01 & -0.03 & 0.01 & 0.05 & 0.08 & -0.03 & -0.03 & -0.01 & 0.04 & 0.06 & -0.03 & 0.05 & 0.03 & -0.04 & -0.01 & 0.00 & -0.01 & 0.01 & -0.03 & 0.01 & -0.02 & 0.02 & 0.05 & 0.08 & 0.04 & 0.08 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  \\ 
   \bottomrule
\end{tabular}
\endgroup
\end{table*}
